The Cosmic Dawn and Epoch of Reionization with the Square Kilometre Array

Concerted effort is currently ongoing to open up the Epoch of Reionization (EoR) ($z\sim$15-6) for studies with IR and radio telescopes. Whereas IR detections have been made of sources (Lyman-$\alpha$ emitters, quasars and drop-outs) in this redshift regime in relatively small fields of view, no direct detection of neutral hydrogen, via the redshifted 21-cm line, has yet been established. Such a direct detection is expected in the coming years, with ongoing surveys, and could open up the entire universe from $z\sim$6-200 for astrophysical and cosmological studies, opening not only the EoR, but also its preceding Cosmic Dawn ($z\sim$30-15) and possibly even the later phases of the Dark Ages ($z\sim$200-30). All currently ongoing experiments attempt statistical detections of the 21-cm signal during the EoR, with limited signal-to-noise. Direct imaging, except maybe on the largest (degree) scales at lower redshifts, as well as higher redshifts will remain out of reach. The Square Kilometre Array(SKA) will revolutionize the field, allowing direct imaging of neutral hydrogen from scales of arc-minutes to degrees over most of the redshift range $z\sim$6-28 with SKA1-LOW, and possibly even higher redshifts with the SKA2-LOW. In this SKA will be unique, and in parallel provide enormous potential of synergy with other upcoming facilities (e.g. JWST). In this chapter we summarize the physics of 21-cm emission, the different phases the universe is thought to go through, and the observables that the SKA can probe, referring where needed to detailed chapters in this volume (Abridged).

==> authors.tex <==
% Author list with institions, for appendix
% Institution should be brief (single line!), with country
% Examples for Koopmans, Pritchard and Mellema are shown
\appendix
\section{Author Institions}
\noindent

L.V.E Koopmans,
Kapteyn Astronomical Institute, University of Groningen, The Netherlands\\
J.~Pritchard, Imperial College, U.K.\\
G.~Mellema, Stockholm Univ., Sweden\\
F.~Abdalla, 
J.~Aguirre, 
K.~Ahn, 
R.~Barkana, 
I.~van Bemmel, 
G.~Bernardi, 
A.~Bonaldi,
F.~Briggs, 
A.G.~de Bruyn, 
T.C.~Chang, 
E.~Chapman, 
X.~Chen, 
J.~Chengalur, 
B.~Ciardi,  
K.K.~Datta, 
P.~Dayal, 
A.~Ferrara, 
A.~Fialkov, 
F.~Fiore, 
K.~Ichiki, 
I.~Illiev, 
S.~Inoue, 
V.~Jelic, 
M.~Jones, 
J.~Lazio, 
U.~Maio, 
S.~Majumdar, 
A.~Mesinger, 
M.~Morales,  
A.~Parsons, 
U.-L.~Pen, 
M.~Santos, 
R.~Schneider, 
B.~Semelin,  
R.~Subrahmanyan, 
T.~Takeuchi, 
C.~Trott, 
H.~Vedantham, 
R.~Webster, 
S.~Wyithe, 
R.S.~de Zouza

% END

